Data-Efficient Training of CNNs and Transformers with Coresets: A Stability Perspective

Coreset selection is among the most effective ways to reduce the training time of CNNs, however, only limited is known on how the resultant models will behave under variations of the coreset size, and choice of datasets and models. Moreover, given the recent paradigm shift towards transformer-based models, it is still an open question how coreset selection would impact their performance. There are several similar intriguing questions that need to be answered for a wide acceptance of coreset selection methods, and this paper attempts to answer some of these. We present a systematic benchmarking setup and perform a rigorous comparison of different coreset selection methods on CNNs and transformers. Our investigation reveals that under certain circumstances, random selection of subsets is more robust and stable when compared with the SOTA selection methods. We demonstrate that the conventional concept of uniform subset sampling across the various classes of the data is not the appropriate choice. Rather samples should be adaptively chosen based on the complexity of the data distribution for each class. Transformers are generally pretrained on large datasets, and we show that for certain target datasets, it helps to keep their performance stable at even very small coreset sizes. We further show that when no pretraining is done or when the pretrained transformer models are used with non-natural images (e.g. medical data), CNNs tend to generalize better than transformers at even very small coreset sizes. Lastly, we demonstrate that in the absence of the right pretraining, CNNs are better at learning the semantic coherence between spatially distant objects within an image, and these tend to outperform transformers at almost all choices of the coreset size.

==> benchmarking.tex <==
\subsection{Benchmarking strategy}
For a fair comparison of different coreset selection methods across the different CNN and transformer methods, we define here a benchmarking setup. Note that this setup is designed with respect to making the training process more efficient. In this regard, we first introduce some parameters that will be used consistently across all experiments of this paper to compare the results. Following this, we describe the setup that we use for the purpose of benchmarking.

\textbf{Definitions. }There are several parameters that control parameters that are important for the setup and we define them here. Together with the definition, we also provide the motivation behind the relevance of each of the introduced parameters in the context of comparing various coreset methods for CNNs and transformers across different coreset sizes.

\textit{Effective data per epoch (EDPE). } It refers to the fraction of the trainset used as coreset for training the model per epoch. EDPE gives an approximate estimate of the reduction in the training time of the model.

\textit{Subset selection interval (SSI). }It refers to the number of epochs that need to be run before two consecutive coreset selections. Thus, for a setup with a fixed number of epochs, a higher value of SSI would imply a lesser number of coreset selection cycles. In general, the influence of SSI is not well known on the overall performance of the trained model, and we experiment with different values of SSI to find the right number of coreset selections that maximize the model performance. 

\textit{Total selection time. }It refers to the amount of time spent on selecting the optimal subset of the training data using the chosen coreset selection method. Although it is assumed that the cost associated with coreset selection is negligible, 

\textit{Total time. }It corresponds to the total time spent on training the model as well as coreset selection. In terms of computing the efficiency of a training process, we consider total time as the right metric and report it frequently in our results presented later in this paper.

\textit{Epochs. }Similar to any training procedure in deep learning, epoch refers to the number of passes through the entire dataset (coreset here). It can also be interpreted as the iterative effort invested to identify the best model and has a significant impact on the training cost. Note that best models for different methods might be obtained at a different epoch value, however, when calculating the training cost, we consider the total number of epochs that are planned beforehand. The reason is that from the implementation perspective, the best model cannot be known till the model has


==> discuss.tex <==

\textit{Adaptation for transformers. }



==> plots/c10/craig/4subplot/a.tex <==
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
    xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=270,
    ymin=20, ymax=70,
    xtick={0,30, 60, 90, 120, 150, 180, 210, 240, 270},
    ytick={0, 20, 30, 40, 50, 60, 70},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=star,
    dashed,
    ]
    coordinates {
    (30.38,32.73)
    (54.29,51.99)
    (75.67,52.26)
    (99.90,57.75)
    (125.13,59.28)
    (148.45,61.15)
    (171.45,61.70)
    (196.18,63.77)
    (217.94,65.42)
    (240.75,66.66)
    };
    \addlegendentry{Craig-10}

\addplot[
    color=blue,
    mark=star,
    dotted,
    ]
    coordinates {
    (16.49,33.24)
    (39.01,51.59)
    (60.52,55.58)
    (87.05,57.67)
    (109.69,60.17)
    (132.09,61.44)
    (156.75,62.56)
    (181.35,63.53)
    (201.95,65.82)
    (227.10,66.76)
    };
    \addlegendentry{Craig-20}

\addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (8.02,33.04)
    (29.24,50.57)
    (52.25,53.70)
    (78.51,57.79)
    (100.47,60.10)
    (122.60,62.02)
    (147.65,63.12)
    (170.78,64.88)
    (193.10,66.44)
    (217.38,67.03)
    };
    \addlegendentry{Craig-50}

\addplot[
    color=red,
    mark=star,
    dashed,
    ]
    coordinates {
    (27.15,27.77)
    (48.38,50.53)
    (138.02,62.90)
    (209.07,66.79)
    % (125.13,59.28)
    % (148.45,61.15)
    % (171.45,61.70)
    % (196.18,63.77)
    % (217.94,65.42)
    % (240.75,66.66)
    };
    \addlegendentry{GradMatch-10}

\addplot[
    color=red,
    mark=star,
    dotted,
    ]
    coordinates {
    (14.95,27.55)
    (35.97,50.16)
    (123.88,63.56)
    (193.99,67.05)
    % (109.69,60.17)
    % (132.09,61.44)
    % (156.75,62.56)
    % (181.35,63.53)
    % (201.95,65.82)
    % (227.10,66.76)
    };
    \addlegendentry{GradMatch-20}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (7.25,30.00)
    (28.16,49.04)
    (116.13,63.53)
    (183.22,67.22)
    % (100.47,60.10)
    % (122.60,62.02)
    % (147.65,63.12)
    % (170.78,64.88)
    % (193.10,66.44)
    % (217.38,67.03)
    };
    \addlegendentry{GradMatch-50}
\end{axis}
\end{tikzpicture}


==> plots/c10/craig/4subplot/b.tex <==
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
    xlabel={Effective Data Per Epoch[\%]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=100,
    ymin=20, ymax=70,
    xtick={1, 10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick={0, 20, 30, 40, 50, 60, 70},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=star,
    dashed,
    ]
    coordinates {
    (1,32.73)
    (10,51.99)
    (20,52.26)
    (30,57.75)
    (40,59.28)
    (50,61.15)
    (60,61.70)
    (70,63.77)
    (80,65.42)
    (90,66.66)
    };
    \addlegendentry{{Craig-10}

\addplot[
    color=blue,
    mark=star,
    dotted,
    ]
    coordinates {
    (1,33.24)
    (10,51.59)
    (20,55.58)
    (30,57.67)
    (40,60.17)
    (50,61.44)
    (60,62.56)
    (70,63.53)
    (80,65.82)
    (90,66.76)
    };
    \addlegendentry{{Craig-20}

\addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (1,33.04)
    (10,50.57)
    (20,53.70)
    (30,57.79)
    (40,60.10)
    (50,62.02)
    (60,63.12)
    (70,64.88)
    (80,66.44)
    (90,67.03)
    };
    \addlegendentry{{Craig-50}

\addplot[
    color=red,
    mark=star,
    dashed,
    ]
    coordinates {
    (1,27.77)
    (10,50.53)
    (50,62.90)
    (80,66.79)
    % (125.13,59.28)
    % (148.45,61.15)
    % (171.45,61.70)
    % (196.18,63.77)
    % (217.94,65.42)
    % (240.75,66.66)
    };
    \addlegendentry{GradMatch-10}

\addplot[
    color=red,
    mark=star,
    dotted,
    ]
    coordinates {
    (1,27.55)
    (10,50.16)
    (50,63.56)
    (80,67.05)
    % (109.69,60.17)
    % (132.09,61.44)
    % (156.75,62.56)
    % (181.35,63.53)
    % (201.95,65.82)
    % (227.10,66.76)
    };
    \addlegendentry{GradMatch-20}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (1,30.00)
    (10,49.04)
    (50,63.53)
    (80,67.22)
    % (100.47,60.10)
    % (122.60,62.02)
    % (147.65,63.12)
    % (170.78,64.88)
    % (193.10,66.44)
    % (217.38,67.03)
    };
    \addlegendentry{GradMatch-50}
\end{axis}
\end{tikzpicture}



==> plots/c10/craig/4subplot/c.tex <==
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
    xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=160,
    ymin=15, ymax=95,
    xtick={0,10, 40, 70, 100, 130, 160},
    ytick={0, 15, 25, 35, 45, 55, 65, 75, 85, 95},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=star,
    dashed,
    ]
    coordinates {
    (14.30,27.29)
    (27.07,63.40)
    (42.39,73.00)
    (55.72,78.02)
    (72.94,80.91)
    (84.95,83.31)
    (102.69,86.14)
    (118.97,87.31)
    (130.57,88.70)
    (152.17,89.59)
    };
    \addlegendentry{Craig-10}

\addplot[
    color=blue,
    mark=star,
    dotted,
    ]
    coordinates {
    (7.87,27.72)
    (20.67,62.56)
    (34.51,72.28)
    (49.19,77.77)
    (64.51,80.98)
    (77.55,83.70)
    (96.62,86.01)
    (113.80,87.38)
    (118.59,89.06)
    (144.45,89.46)
    };
    \addlegendentry{Craig-20}

\addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (4.13,28.98)
    (17.29,61.27)
    (31.11,71.22)
    (46.30,77.76)
    (61.54,81.99)
    (75.40,84.60)
    (91.03,86.79)
    (107.29,87.97)
    (120.97,89.33)
    (134.64,89.64)
    };
    \addlegendentry{Craig-50}

    \addplot[
    color=red,
    mark=star,
    dashed,
    ]
    coordinates {
    (11.31,23.74)
    (30.69,63.91)
    (82.37,86.81)
    (124.89,89.55)
    % (72.94,80.91)
    % (84.95,83.31)
    % (102.69,86.14)
    % (118.97,87.31)
    % (130.57,88.70)
    % (152.17,89.59)
    };
    \addlegendentry{GradMatch-10}

\addplot[
    color=red,
    mark=star,
    dotted,
    ]
    coordinates {
    (6.65,24.92)
    (23.33,64.35)
    (77.27,86.26)
    (119.48,89.78)
    % (64.51,80.98)
    % (77.55,83.70)
    % (96.62,86.01)
    % (113.80,87.38)
    % (118.59,89.06)
    % (144.45,89.46)
    };
    \addlegendentry{GradMatch-20}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (3.62,27.15)
    (18.57,60.61)
    (73.27,85.09)
    (115.79,89.55)
    % (61.54,81.99)
    % (75.40,84.60)
    % (91.03,86.79)
    % (107.29,87.97)
    % (120.97,89.33)
    % (134.64,89.64)
    };
    \addlegendentry{GradMatch-50}
    
\end{axis}
\end{tikzpicture}



==> plots/c10/craig/4subplot/d.tex <==
\begin{tikzpicture}[scale=0.5]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
    xlabel={Effective Data per Epoch [\%]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=100,
    ymin=15, ymax=95,
    xtick={1,10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
    ytick={0, 15, 25, 35, 45, 55, 65, 75, 85, 95},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=star,
    dashed,
    ]
    coordinates {
    (1,27.29)
    (10,63.40)
    (20,73.00)
    (30,78.02)
    (40,80.91)
    (50,83.31)
    (60,86.14)
    (70,87.31)
    (80,88.70)
    (90,89.59)
    };
    \addlegendentry{Craig-10}

\addplot[
    color=blue,
    mark=star,
    dotted,
    ]
    coordinates {
    (1,27.72)
    (10,62.56)
    (20,72.28)
    (30,77.77)
    (40,80.98)
    (50,83.70)
    (60,86.01)
    (70,87.38)
    (80,89.06)
    (90,89.46)
    };
    \addlegendentry{Craig-20}

\addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (1,28.98)
    (10,61.27)
    (20,71.22)
    (30,77.76)
    (40,81.99)
    (50,84.60)
    (60,86.79)
    (70,87.97)
    (80,89.33)
    (90,89.64)
    };
    \addlegendentry{Craig-50}

    \addplot[
    color=red,
    mark=star,
    dashed,
    ]
    coordinates {
    (1,23.74)
    (10,63.91)
    (50,86.81)
    (80,89.55)
    % (72.94,80.91)
    % (84.95,83.31)
    % (102.69,86.14)
    % (118.97,87.31)
    % (130.57,88.70)
    % (152.17,89.59)
    };
    \addlegendentry{GradMatch-10}

\addplot[
    color=red,
    mark=star,
    dotted,
    ]
    coordinates {
    (1,24.92)
    (10,64.35)
    (50,86.26)
    (80,89.78)
    % (64.51,80.98)
    % (77.55,83.70)
    % (96.62,86.01)
    % (113.80,87.38)
    % (118.59,89.06)
    % (144.45,89.46)
    };
    \addlegendentry{GradMatch-20}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (1,27.15)
    (10,60.61)
    (50,85.09)
    (80,89.55)
    % (61.54,81.99)
    % (75.40,84.60)
    % (91.03,86.79)
    % (107.29,87.97)
    % (120.97,89.33)
    % (134.64,89.64)
    };
    \addlegendentry{GradMatch-50}
    
\end{axis}
\end{tikzpicture}



==> plots/c10/craig/4subplot/plot.tex <==
\begin{figure}
        \centering
        \begin{subfigure}[b]{0.3\textwidth}
            \centering
            \input{plots/c10/craig/4subplot/a.tex}
            \caption[Network2]%
            {{\small ViT\_B16 performance}}    
            \label{fig:mean and std of net14}
        \end{subfigure}
        % \hskip 5pt
        \begin{subfigure}[b]{0.3\textwidth}  
            \centering 
            \input{plots/c10/craig/4subplot/b.tex}
            \caption[]%
            {{\small ViT\_B16 performance}}    
            \label{fig:mean and std of net24}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.3\textwidth}   
            \centering 
            \input{plots/c10/craig/4subplot/c.tex}
            \caption[]%
            {{\small ResNet50V2 performance}}    
            \label{fig:mean and std of net34}
        \end{subfigure}
        % \hskip 5pt
        \begin{subfigure}[b]{0.3\textwidth}   
            \centering 
            \input{plots/c10/craig/4subplot/d.tex}
            \caption[]%
            {{\small ResNet50V2 performance}}    
            \label{fig:mean and std of net44}
        \end{subfigure}
        \caption[]
        {\small Performance comparsion between random intialized ViT\_B16 and ResNet50v2 on CIFAR10 Method=Craig } 
        \label{fig:mean and std of nets}
    \end{figure}



% \begin{figure}[h]
%     \centering
%   \begin{tikzpicture}
%     \begin{groupplot}[
%       group style={group size=2 by 2},
%       width=5cm, height=5cm,
%     ]
%     \nextgroupplot[
%     % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
%     xlabel={Time [Mins]},
%     ylabel={Accuracy [\%]},
%     xmin=0, xmax=270,
%     ymin=30, ymax=70,
%     xtick={0,30, 60, 90, 120, 150, 180, 210, 240, 270},
%     ytick={0, 30, 40, 50, 60, 70},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
%     line width=1pt
% ]
    
%       \addplot[
%     color=blue,
%     mark=star,
%     dashed,
%     ]
%     coordinates {
%     (30.38,32.73)
%     (54.29,51.99)
%     (75.67,52.26)
%     (99.90,57.75)
%     (125.13,59.28)
%     (148.45,61.15)
%     (171.45,61.70)
%     (196.18,63.77)
%     (217.94,65.42)
%     (240.75,66.66)
%     };
%     \addlegendentry{ViT\_B16-10}

% \addplot[
%     color=blue,
%     mark=star,
%     dotted,
%     ]
%     coordinates {
%     (16.49,33.24)
%     (39.01,51.59)
%     (60.52,55.58)
%     (87.05,57.67)
%     (109.69,60.17)
%     (132.09,61.44)
%     (156.75,62.56)
%     (181.35,63.53)
%     (201.95,65.82)
%     (227.10,66.76)
%     };
%     \addlegendentry{ViT\_B16-20}

% \addplot[
%     color=blue,
%     mark=star,
%     ]
%     coordinates {
%     (8.02,33.04)
%     (29.24,50.57)
%     (52.25,53.70)
%     (78.51,57.79)
%     (100.47,60.10)
%     (122.60,62.02)
%     (147.65,63.12)
%     (170.78,64.88)
%     (193.10,66.44)
%     (217.38,67.03)
%     };
%     \addlegendentry{ViT\_B16-50}
    
%     \nextgroupplot[
%     % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
%     xlabel={Effective Data Per Epoch[\%]},
%     ylabel={Accuracy [\%]},
%     xmin=0, xmax=100,
%     ymin=30, ymax=70,
%     xtick={0,1, 10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
%     ytick={0, 30, 40, 50, 60, 70},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
%     line width=1pt
% ]
%      \addplot[
%     color=blue,
%     mark=star,
%     dashed,
%     ]
%     coordinates {
%     (1,32.73)
%     (10,51.99)
%     (20,52.26)
%     (30,57.75)
%     (40,59.28)
%     (50,61.15)
%     (60,61.70)
%     (70,63.77)
%     (80,65.42)
%     (90,66.66)
%     };
%     \addlegendentry{ViT\_B16-10}

% \addplot[
%     color=blue,
%     mark=star,
%     dotted,
%     ]
%     coordinates {
%     (1,33.24)
%     (10,51.59)
%     (20,55.58)
%     (30,57.67)
%     (40,60.17)
%     (50,61.44)
%     (60,62.56)
%     (70,63.53)
%     (80,65.82)
%     (90,66.76)
%     };
%     \addlegendentry{ViT\_B16-20}

% \addplot[
%     color=blue,
%     mark=star,
%     ]
%     coordinates {
%     (1,33.04)
%     (10,50.57)
%     (20,53.70)
%     (30,57.79)
%     (40,60.10)
%     (50,62.02)
%     (60,63.12)
%     (70,64.88)
%     (80,66.44)
%     (90,67.03)
%     };
%     \addlegendentry{ViT\_B16-50}
%     \nextgroupplot[
%     % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
%     xlabel={Time [Mins]},
%     ylabel={Accuracy [\%]},
%     xmin=0, xmax=160,
%     ymin=25, ymax=95,
%     xtick={0,10, 40, 70, 100, 130, 160},
%     ytick={0, 25, 35, 45, 55, 65, 75, 85, 95},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
%     line width=1pt
% ]
%       \addplot[
%     color=red,
%     mark=otimes,
%     dashed,
%     ]
%     coordinates {
%     (14.30,27.29)
%     (27.07,63.40)
%     (42.39,73.00)
%     (55.72,78.02)
%     (72.94,80.91)
%     (84.95,83.31)
%     (102.69,86.14)
%     (118.97,87.31)
%     (130.57,88.70)
%     (152.17,89.59)
%     };
%     \addlegendentry{ResNet50v2-10}

% \addplot[
%     color=red,
%     mark=otimes,
%     dotted,
%     ]
%     coordinates {
%     (7.87,27.72)
%     (20.67,62.56)
%     (34.51,72.28)
%     (49.19,77.77)
%     (64.51,80.98)
%     (77.55,83.70)
%     (96.62,86.01)
%     (113.80,87.38)
%     (118.59,89.06)
%     (144.45,89.46)
%     };
%     \addlegendentry{ResNet50v2-20}

% \addplot[
%     color=red,
%     mark=otimes,
%     ]
%     coordinates {
%     (4.13,28.98)
%     (17.29,61.27)
%     (31.11,71.22)
%     (46.30,77.76)
%     (61.54,81.99)
%     (75.40,84.60)
%     (91.03,86.79)
%     (107.29,87.97)
%     (120.97,89.33)
%     (134.64,89.64)
%     };
%     \addlegendentry{ResNet50v2-50}
%       \nextgroupplot[
%     % title={Performance comparison between ViT\_B16 and ResNetV2-50 for time and performance},
%     xlabel={Effective Data per Epoch [\%]},
%     ylabel={Accuracy [\%]},
%     xmin=0, xmax=100,
%     ymin=25, ymax=95,
%     xtick={0,10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
%     ytick={0, 25, 35, 45, 55, 65, 75, 85, 95},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
%     line width=1pt
% ]
%      \addplot[
%     color=red,
%     mark=otimes,
%     dashed,
%     ]
%     coordinates {
%     (1,27.29)
%     (10,63.40)
%     (20,73.00)
%     (30,78.02)
%     (40,80.91)
%     (50,83.31)
%     (60,86.14)
%     (70,87.31)
%     (80,88.70)
%     (90,89.59)
%     };
%     \addlegendentry{ResNet50v2-10}

% \addplot[
%     color=red,
%     mark=otimes,
%     dotted,
%     ]
%     coordinates {
%     (1,27.72)
%     (10,62.56)
%     (20,72.28)
%     (30,77.77)
%     (40,80.98)
%     (50,83.70)
%     (60,86.01)
%     (70,87.38)
%     (80,89.06)
%     (90,89.46)
%     };
%     \addlegendentry{ResNet50v2-20}

% \addplot[
%     color=red,
%     mark=otimes,
%     ]
%     coordinates {
%     (1,28.98)
%     (10,61.27)
%     (20,71.22)
%     (30,77.76)
%     (40,81.99)
%     (50,84.60)
%     (60,86.79)
%     (70,87.97)
%     (80,89.33)
%     (90,89.64)
%     };
%     \addlegendentry{ResNet50v2-50}
    
%     \end{groupplot}
%   \end{tikzpicture}

%   \caption{Performance comparison between ViT\_B16 and ResNetV2-50 with ImageNet21k weights Initialization for time and performance for CIFAR10, Method=Craig}
% \label{fig:fig3}
% \end{figure}

==> plots/imgnet/craig/10-3models.tex <==
% \begin{flushed left}
\begin{figure}[h]
    \centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 with ImageNet21k weights Initialization for time and performance for Tiny ImageNet, Method=Craig},
    xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=100, xmax=600,
    ymin=15, ymax=95,
    xtick={100, 200, 300, 400, 500, 600},
    ytick={15, 25, 35, 45, 55, 65, 75, 85, 95},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (191.59,48.30)
    (235.84, 84.97)
    (332.62,88.48)
    (429.41,89.97)
    (575.97,89.46)
    % (833.88,90.12)
    };
    \node [right] at (axis cs:  191.59,48.30) {$1\%$};
    \node [left] at (axis cs:  235.84, 84.97) {$10\%$};
    \node [above] at (axis cs:  332.62,88.48) {$30\%$};
    \node [below] at (axis cs:  429.41,89.97) {$50\%$};
    \node [below] at (axis cs:  575.97,89.46) {$80\%$};
    \addlegendentry{ViT\_B16}

\addplot[
    color=red,
    mark=diamond,
    ]
    coordinates {
    (140.30, 60.83)
    (168.94, 72.21)
    (231.58, 78.94)
    (294.23, 80.87)
    (389.09, 79.76)};
    % \node [left] at (axis cs:  140.30, 60.83) {$1\%$};
    % \node [left] at (axis cs:  168.94, 72.21) {$10\%$};
    % \node [above] at (axis cs: 231.58, 78.94) {$30\%$};
    % \node [below] at (axis cs: 294.23, 80.87) {$50\%$};
    % \node [below] at (axis cs: 389.09, 79.76) {$80\%$};
    \addlegendentry{ResNet50V2}

\addplot[
    color=violet,
    mark=pentagon,
    ]
    coordinates {
    (165.27, 17.15)
    (192.15, 59.15)
    (250.97, 72.10)
    (309.78, 75.35)
    (398.84, 75.76)};
    % \node [left] at (axis cs:  165.27, 17.15) {$1\%$};
    % \node [right] at (axis cs:  192.15, 59.15) {$10\%$};
    % \node [below] at (axis cs:  250.97, 72.10) {$30\%$};
    % \node [below] at (axis cs:  309.78, 75.35) {$50\%$};
    % \node [below] at (axis cs:  398.84, 75.76) {$80\%$};
    \addlegendentry{MobileNetV3\-Large}

    
    

% \addplot[
%     color=black,
%     mark=triangle,
%     ]
%     coordinates {
%     (5.45, 41.01)
%     (54.57, 87.21)
%     (160.98, 89.21)
%     (267.4, 89.73)
%     (428.39, 89.73)
%     };
%     \addlegendentry{Random}

% \addplot[
%     color=blue,
%     mark=star,
%     ]
%     coordinates {
%     % (0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)
%     (47.45,28.48)(118.31,86.93)(263.64,89.01)(412.36,89.46)(633.50,89.85)
%     };
%     \addlegendentry{ViT\_B16-50}

% \addplot[
%     color=red,
%     mark=x,
%     ]
%     coordinates {
%     % (0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)
%     (225.98,56.76)(241.80,72.09)(305.72,76.47)(374.29,79.13)(474.19,79.21)
%     };
%     \addlegendentry{ResNetv2-50-10}

% \addplot[
%     color=red,
%     mark=star,
%     ]
%     coordinates {
%     % (0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)
%     (105.59,53.58)(129.83,72.09)(197.71,77.30)(266.11,79.77)(369.26,78.56)
%     };
%     \addlegendentry{ResNetv2-50-pretrained-20}

% \addplot[
%     color=red,
%     mark=otimes,
%     ]
%     coordinates {
%     % (0,23.1)(10,27.5)(20,32)(30,37.8)(40,44.6)(60,61.8)(80,83.8)(100,114)
%     (43.82,51.35)(70.16,72.13)(145.08,76.84)(210.76,77.92)(322.89,78.22)
%     };
%     \addlegendentry{ResNetv2-50-pretrained-50}
    
\end{axis}
\end{tikzpicture}
\caption{Performance comparison between different backbones with pretrained weights Initialization for time and performance on Tiny ImageNet, Method=Craig, SSI=10. As the subset size is increased, final accuracy increases accordingly. Size of the subset is labelled in ViT results and same subset size pattern is followed in other backbones.}
\label{fig:fig4}
\end{figure}


==> plots/imgnet/craig/ssi-vit.tex <==
\begin{figure}
        \centering
\begin{tikzpicture}[scale=0.48]
   \begin{axis}[ xlabel={Time [mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=600,
    ymin=25, ymax=95,
   xtick={0, 150, 300, 450, 600},
    ytick={0, 25, 35, 45, 55, 65, 75, 85, 95},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt,
    legend style={nodes={scale=1.2, transform shape}}
    ]
\addplot[
    color=blue,
    mark=star,
    dashed
    ]
    coordinates {
    (191.59,48.30)
    (235.84, 84.97)
    (332.62,88.48)
    (429.41,89.97)
    (575.97,89.46)
    };
    \addlegendentry{SSI-10}

\addplot[
    color=blue,
    mark=star,
    dotted
    ]
    coordinates {
    (191.59,39.39)
    (235.84, 84.46)
    (332.62,89.05)
    (429.41,89.59)
    (575.97,89.28)
    };
    \addlegendentry{SSI-20}

    \addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
   (191.59,33.73)
    (235.84, 86.00)
    (332.62,89.01)
    (429.41,89.18)
    (575.97,89.23)
    };
    \addlegendentry{SSI-50}

%     \addplot[
%     color=red,
%     mark=star,
%     dotted
%     ]
%     coordinates {
%     (1,27.15)
%     (10,60.61)
%     (50,85.09)
%     (80,89.55)
%     % (61.54,81.99)
%     % (75.40,84.60)
%     % (91.03,86.79)
%     % (107.29,87.97)
%     % (120.97,89.33)
%     % (134.64,89.64)
%     };
%     \addlegendentry{ResNet50v2-GradMatch-50}
%     \end{axis}
%     \end{tikzpicture}%
%     ~%
%     %
%     \begin{tikzpicture}[ scale=0.48]
%     \begin{axis}[ xlabel={Time [Mins]},
%     ylabel={Accuracy [\%]},
%     xmin=0, xmax=245,
%     ymin=25, ymax=95,
%     xtick={5, 35, 65, 95, 125, 155, 185, 215, 245},
%     ytick={0, 25, 35, 45, 55, 65, 75, 85, 95},
%     legend pos=south east,
%     ymajorgrids=true,
%     grid style=dashed,
%     line width=1pt,    
%     ]
% \addplot[
%     color=blue,
%     mark=star,
%     dashed
%     ]
%     coordinates {
%     (8.02,33.04)
%     (29.24,50.57)
%     (52.25,53.70)
%     (78.51,57.79)
%     (100.47,60.10)
%     (122.60,62.02)
%     (147.65,63.12)
%     (170.78,64.88)
%     (193.10,66.44)
%     (217.38,67.03)
%     };
%     \addlegendentry{ViT\_B16-Craig-50}

% \addplot[
%     color=blue,
%     mark=star,
%     dotted
%     ]
%     coordinates {
%     (7.25,30.00)
%     (28.16,49.04)
%     (116.13,63.53)
%     (183.22,67.22)
%     % (100.47,60.10)
%     % (122.60,62.02)
%     % (147.65,63.12)
%     % (170.78,64.88)
%     % (193.10,66.44)
%     % (217.38,67.03)
%     };
%     \addlegendentry{ViT\_B16-GradMatch-50}

% \addplot[
%     color=red,
%     mark=star,
%     dashed
%     ]
%     coordinates {
%     (4.13,28.98)
%     (17.29,61.27)
%     (31.11,71.22)
%     (46.30,77.76)
%     (61.54,81.99)
%     (75.40,84.60)
%     (91.03,86.79)
%     (107.29,87.97)
%     (120.97,89.33)
%     (134.64,89.64)
%     };
%     \addlegendentry{ResNet50V2-Craig-50}

%     \addplot[
%     color=red,
%     mark=star,
%     dotted
%     ]
%     coordinates {
%     (3.62,27.15)
%     (18.57,60.61)
%     (73.27,85.09)
%     (115.79,89.55)
%     % (61.54,81.99)
%     % (75.40,84.60)
%     % (91.03,86.79)
%     % (107.29,87.97)
%     % (120.97,89.33)
%     % (134.64,89.64)
%     };
%     \addlegendentry{ResNet50V2-GradMatch-50}
    \end{axis}
    \end{tikzpicture}%
\vspace{-1em}
\caption{Performance comparison with varying SSI on ViT\_B16 and keeping time constant on Tiny ImageNet, Method=Craig}
\label{fig:fig3}
\end{figure}

==> plots/imgnet/r50v2_imgnet_methods.tex <==
% \begin{flushed left}
\begin{figure}[h]
    \centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 with ImageNet21k weights Initialization for time and performance for Tiny ImageNet, Method=Craig},
    xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=400,
    ymin=40, ymax=85,
    xtick={0, 3, 50, 100, 150, 200, 250, 300, 350, 400},
    ytick={40, 45, 50, 55, 60, 65, 70, 75, 80, 85},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (30.60, 49.00)
    (59.24, 73.18)
    (121.89, 77.71)
    (184.53, 78.89)
    (279.40, 79.16)};
    \addlegendentry{Craig}

\addplot[
    color=red,
    mark=diamond,
    ]
    coordinates {
    (19.15, 60.88)
    (46.75, 75.36)
    (107.13, 77.74)
    (167.51, 78.61)
    (258.94, 79.16)};
    \addlegendentry{GradMatch}

\addplot[
    color=violet,
    mark=pentagon,
    ]
    coordinates {
   (15.82, 57.57)
    (44.07, 71.22)
    (104.11, 75.55)
    (167.68, 78.11)
    (259.50, 79.09)};
    \addlegendentry{Glister}

    
    

\addplot[
    color=black,
    mark=triangle,
    ]
    coordinates {
    (3.53, 56.76)
    (31.78, 71.51)
    (95.35, 75.59)
    (155.38, 78.17)
    (250.73, 78.81)
    };
    \addlegendentry{Random}

\end{axis}
\end{tikzpicture}
\caption{Performance comparison between different subsets methods with BiT-M-R50x1 on ImageNet21k weights Initialization for time and performance on Tiny ImageNet, SSI=50}
\label{fig:r50v2-subsets}
\end{figure}


==> plots/imgnet/subset_comp_vit.tex <==
\begin{figure}
        \centering
\begin{tikzpicture}[scale=0.48]
   \begin{axis}[ xlabel={Training Time [Mins]},
    ylabel={Accuracy [\%]},
   xmin=0, xmax=280,
    ymin=15, ymax=85,
    xtick={3, 40, 80, 120, 160, 200, 240, 280},
    ytick={15, 25, 35, 45, 55, 65, 75, 85},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt,
    ]
 \addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (191.59,48.30)
    (235.84, 84.97)
    (332.62,88.48)
    (429.41,89.97)
    (575.97,89.46)};
    \addlegendentry{CRAIG-ViT\_B16}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (124.68, 60.66)
    (174.09, 88.21)
    (281.28, 90.03)
    (396.35, 90.27)
    (549.17, 90.22)};
    \addlegendentry{GradMatch-ViT\_B16}

\addplot[
    color=violet,
    mark=star,
    ]
    coordinates {
    (87.18, 55.03)
    (137.54, 88.62)
    (160.98, 89.21)
    (267.4, 89.73)
    (428.39, 89.73)};
    \addlegendentry{Glister-ViT\_B16}

    \addplot[
        color=black,
        mark=star,
        ]
        coordinates {
        (5.45, 41.01)
        (54.57, 87.21)
        (160.98, 89.21)
        (267.4, 89.73)
        (428.39, 89.73)
        };
        \addlegendentry{Random-ViT\_B16}

    \addplot[
    color=blue,
    mark=star,
    dashed
    ]
    coordinates {
    (3.36,17.15)
    (30.24, 59.15)
    (89.05,72.10)
    (147.87,75.35)
    (236.92,75.76)};
    \addlegendentry{CRAIG-MobileNetV3-large}

\addplot[
    color=red,
    mark=star,
    dashed
    ]
    coordinates {
    (3.36, 29.35)
    (30.24, 72.42)
    (89.05, 75.47)
    (147.87, 75.75)
    (236.92, 75.39)};
    \addlegendentry{GradMatch-MobileNetV3-large}

\addplot[
    color=violet,
    mark=star,
    dashed
    ]
    coordinates {
    (3.36, 20.68)
    (30.24, 68.37)
    (89.05, 75.15)
    (147.87, 75.45)
    (236.92, 75.87)};
    \addlegendentry{Glister-MobileNetV3-large}

    
    

    \addplot[
        color=black,
        mark=star,
        dashed
        ]
        coordinates {
        (3.36, 22.72)
        (30.24, 62.58)
        (89.05, 70.60)
        (147.87, 72.34)
        (236.92, 74.44)
        };
        \addlegendentry{Random-MobileNetV3-large}
    \end{axis}
    \end{tikzpicture}%
    ~%
    %
    \begin{tikzpicture}[ scale=0.48]
    \begin{axis}[ xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=420,
    ymin=15, ymax=85,
    xtick={3, 60, 120, 180, 240, 300, 360, 420},
    ytick={15, 25, 35, 45, 55, 65, 75, 85},
    % legend pos=outer north east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt,    
    ]
\addplot[
    color=blue,
    mark=star,
    ]
    coordinates {
    (140.30,60.83)
    (168.94, 72.21)
    (231.58,78.94)
    (294.23,80.87)
    (389.09,79.79)};
    % \addlegendentry{CRAIG-ResNet-50x1}

\addplot[
    color=red,
    mark=star,
    ]
    coordinates {
    (81.42, 72.49)
    (109.02, 80.24)
    (169.40, 81.09)
    (229.79, 80.41)
    (321.22, 79.40)};
    % \addlegendentry{GradMatch-ResNet-50x1}

\addplot[
    color=violet,
    mark=star,
    ]
    coordinates {
    (66.01, 63.99)
    (94.27, 75.08)
    (154.30, 76.73)
    (217.87, 78.11)
    (309.69, 79.09)};
    % \addlegendentry{Glister-ResNet-50x1}

    \addplot[
        color=black,
        mark=star,
        ]
        coordinates {
        (3.53, 52.21)
        (31.78, 72.07)
        (95.35, 75.59)
        (155.38, 78.17)
        (250.73, 78.81)
        };
        % \addlegendentry{Random-ResNet-50x1}

    \addplot[
    color=blue,
    mark=star,
    dashed
    ]
    coordinates {
    (165.27,17.15)
    (192.15, 59.15)
    (250.97,72.10)
    (309.78,75.35)
    (398.84,75.76)};
    % \addlegendentry{CRAIG-MobileNetV3-large}

\addplot[
    color=red,
    mark=star,
    dashed
    ]
    coordinates {
    (80.91, 29.35)
    (107.79, 72.42)
    (166.60, 75.47)
    (225.42, 75.75)
    (314.47, 75.39)};
    % \addlegendentry{GradMatch-MobileNetV3-large}

\addplot[
    color=violet,
    mark=star,
    dashed
    ]
    coordinates {
    (42.30, 20.68)
    (69.18, 68.37)
    (127.99, 75.15)
    (186.81, 75.45)
    (275.87, 75.87)};
    % \addlegendentry{Glister-MobileNetV3-large}

    
    

\addplot[
    color=black,
    mark=star,
    dashed
    ]
    coordinates {
    (3.36, 22.72)
    (30.24, 62.58)
    (89.05, 70.60)
    (147.87, 72.34)
    (236.92, 74.44)
    };
    % \addlegendentry{Random-MobileNetV3-large}
    \end{axis}
    \end{tikzpicture}%
\vspace{-1em}
\caption{Performance comparison between different subsets methods with different model architectures on ImageNet21k weights Initialization for time and performance on Tiny ImageNet, SSI=10}
\label{fig:sub-comp-res}
\end{figure}



% \begin{figure}
%     \centering
%     \begin{subcaptiongroup}
%     \centering
%     \subcaptionbox{A cat\label{cat}}
%     [.4\textwidth]{\input{cvpr2023-author_kit-v1_1-1/latex/plots/imgnet/r50v2_imgnet_methods.tex}}%
%     \subcaptionbox{An elephant\label{elephant}}
%     [.4\textwidth]{\input{cvpr2023-author_kit-v1_1-1/latex/plots/imgnet/r50v2_imgnet_methods.tex}}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{subcaptiongroup}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}


% \begin{figure}
%   \begin{tikzpicture}
%      \begin{groupplot}[
%         group style={
%            group size=2 by 2,
%            group name=g, % add a name to each axis
%            vertical sep=1cm,
%            horizontal sep=1cm
%         },
%         width=0.2\textwidth,
%         scale only axis,
%         cycle multiindex* list = {
%             very thick\nextlist
%             red\nextlist 
%             only marks\nextlist
%           },
%         title style={
%           text width=6cm,
%           below=14pt,
%           at={(0.5,0)}
%         }
%      ] 
%      \nextgroupplot[title={\subcaption{}}]
%          \addplot {x}; \addplot {x^2};
%      \nextgroupplot[
%           title={\subcaption{}},
%           cycle list = {red, blue}]
%          \addplot {x}; \addplot {x^2};
%      \nextgroupplot[title={\subcaption{}}] \addplot[green] {x}; \addplot {x^2};
%      \nextgroupplot[title={\subcaption{}}] \addplot[green] {x}; \addplot {x^2};
%        \end{groupplot}
%    \end{tikzpicture}
% \vspace{-2em}
% \caption{Main caption}
% \end{figure}

==> plots/imgnet/vit_imgnet_methods.tex <==
% \begin{flushed left}
\begin{figure}[h]
    \centering
\begin{tikzpicture}[scale=0.6]
\begin{axis}[
    % title={Performance comparison between ViT\_B16 and ResNetV2-50 with ImageNet21k weights Initialization for time and performance for Tiny ImageNet, Method=Craig},
    xlabel={Time [Mins]},
    ylabel={Accuracy [\%]},
    xmin=0, xmax=850,
    ymin=40, ymax=100,
    xtick={0,150, 250, 350, 450, 550, 650, 750, 850},
    ytick={40, 50, 60, 70, 80, 90, 100},
    legend pos= south east,
    ymajorgrids=true,
    grid style=dashed,
    line width=1pt
]

\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (191.59,48.30)
    (235.84, 84.97)
    (332.62,88.48)
    (429.41,89.97)
    (575.97,89.46)};
    \addlegendentry{Craig}

\addplot[
    color=red,
    mark=diamond,
    ]
    coordinates {
    (124.68, 60.66)
    (174.09, 88.21)
    (281.28, 90.03)
    (396.35, 90.27)
    (549.17, 90.22)};
    \addlegendentry{GradMatch}

\addplot[
    color=violet,
    mark=pentagon,
    ]
    coordinates {
    (87.18, 55.03)
    (137.54, 88.62)
    (160.98, 89.21)
    (267.4, 89.73)
    (428.39, 89.73)};
    \addlegendentry{Glister}

    
    

\addplot[
    color=black,
    mark=triangle,
    ]
    coordinates {
    (5.45, 41.01)
    (54.57, 87.21)
    (160.98, 89.21)
    (267.4, 89.73)
    (428.39, 89.73)
    };
    \addlegendentry{Random}

\end{axis}
\end{tikzpicture}
\caption{Performance comparison between different subsets methods with ViT\_B16 on ImageNet21k weights Initialization for time and performance on Tiny ImageNet, SSI=10}
\label{fig:vit-subsets}
\end{figure}

